Graphite: GRAPH-Induced feaTure Extraction for Point Cloud Registration

3D Point clouds are a rich source of information that enjoy growing popularity in the vision community. However, due to the sparsity of their representation, learning models based on large point clouds is still a challenge. In this work, we introduce Graphite, a GRAPH-Induced feaTure Extraction pipeline, a simple yet powerful feature transform and keypoint detector. Graphite enables intensive down-sampling of point clouds with keypoint detection accompanied by a descriptor. We construct a generic graph-based learning scheme to describe point cloud regions and extract salient points. To this end, we take advantage of 6D pose information and metric learning to learn robust descriptions and keypoints across different scans. We Reformulate the 3D keypoint pipeline with graph neural networks which allow efficient processing of the point set while boosting its descriptive power which ultimately results in more accurate 3D registrations. We demonstrate our lightweight descriptor on common 3D descriptor matching and point cloud registration benchmarks and achieve comparable results with the state of the art. Describing 100 patches of a point cloud and detecting their keypoints takes only ~0.018 seconds with our proposed network.

==> sections/table_copy.tex <==
\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{l| p{0.15cm}c c c}
\hline
Method & & MSE & RMSE & MAE \\
\hline\hline
\multirow{2}{*}{ICP} & R & 882.5642 & 29.7079 & 23.5572\\
& t & 8.4537 & 2.9075 & 2.4909 \\ 
\hline 
\multirow{2}{*}{Go-ICP} & R & 131.1824 & 11.4534 & 2.5348\\
& t & 0.0531 & 0.2305 & 0.04192 \\
\hline

\multirow{2}{*}{FGR} & R & 607.6948 & 24.6514 & 10.0559\\
& t &  1.1876 & 1.0897 & 0.2739 \\ 
\hline
\multirow{2}{*}{PointNetLK} & R &  256.1555 & 16.0048 & 4.5956\\
& t & 0.0465 & 0.2155 & 0.0565 \\ 
\hline
\multirow{2}{*}{DCP-v1} & R & 6.9265 & 2.6318 & 1.5158\\
& t &   0.0003 & 0.0180 & 0.0169 \\ 
\hline
\multirow{2}{*}{DCP-v2} & R & \textbf{1.1693} & \textbf{1.0813} & 0.7374\\
& t &  \textbf{0.0002} & \textbf{0.0150} & \textbf{0.0105} \\ 
\hline
\multirow{2}{*}{\textbf{Ours}} & R & 17.762033 & 4.2145 & 2.3497\\
& t &  0.3907 & 0.6250 & 0.4416 \\ 
\hline  
\multirow{2}{*}{\textbf{Ours + ICP}} & R & 4.0263 & 2.0065 & \textbf{0.3119}\\
& t &  0.0982 & 0.3134 & 0.0778 \\ 
\hline
\end{tabular}
\end{center}
\caption{Effect of Gaussian noise on point cloud registration on ModelNet40 dataset\label{table:guassian}
}
\end{table}



\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{l |p{0.15cm}c c c}
\hline
Method & & MSE & RMSE & MAE \\
\hline\hline
\multirow{2}{*}{ICP} & R & 892.6011 & 29.8764 & 23.6261\\
& t &  8.6005 & 2.9326 & 2.5191 \\ 
\hline
\multirow{2}{*}{Go-ICP} & R & 192.2586 & 13.8657 & 2.9141\\
& t & 0.0491 & 0.2215 & 0.0621 \\
\hline
\multirow{2}{*}{FGR} & R &  97.0027 & 9.8489 & 1.4454 \\
& t &  0.0182 & 0.1350 & 0.0223 \\ 
\hline
\multirow{2}{*}{PointNetLK} & R & 306.3239 & 17.5021 & 5.2805\\
& t & 0.0784 & 0.2800 & 0.0720 \\ 
\hline
\multirow{2}{*}{DCP-v1} & R & 6.9265 & 2.6318 & 1.5158\\
& t &   0.0003 & 0.0180 & 0.0169 \\ 
\hline
\multirow{2}{*}{DCP-v2} & R &  19.2013 & 4.3819 & 2.6804\\
& t &  \textbf{0.0025} & \textbf{0.0495} & \textbf{0.0359} \\ 
\hline
\multirow{2}{*}{\textbf{Ours}} & R & 7.4387 & 2.7274 & 1.4906\\
& t &  0.3141 & 0.5604 & 0.3836 \\ 
\hline
\multirow{2}{*}{\textbf{Ours + ICP}} & R & \textbf{0.7458} & \textbf{0.8636} & \textbf{0.1123}\\
& t &  0.0872 & 0.2953 & 0.0702 \\ 
\hline
\end{tabular}
\end{center}
\caption{Point cloud registration comparison on ModelNet objects from unseen categories.\label{table:modelnet}}
\end{table}

